Towards Shape Biased Unsupervised Representation Learning for Domain Generalization

It is known that, without awareness of the process, our brain appears to focus on the general shape of objects rather than superficial statistics of context. On the other hand, learning autonomously allows discovering invariant regularities which help generalization. In this work, we propose a learning framework to improve the shape bias property of self-supervised methods. Our method learns semantic and shape biased representations by integrating domain diversification and jigsaw puzzles. The first module enables the model to create a dynamic environment across arbitrary domains and provides a domain exploration vs. exploitation trade-off, while the second module allows the model to explore this environment autonomously. This universal framework does not require prior knowledge of the domain of interest. Extensive experiments are conducted on several domain generalization datasets, namely, PACS, Office-Home, VLCS, and Digits. We show that our framework outperforms state-of-the-art domain generalization methods by a large margin.

==> abstractv1MH.tex <==
\begin{abstract}
   Shape bias plays an important role in self-supervised learning paradigm. The ultimate goal in self-supervised learning is capture a representation that is based as much as possible on the semantic of objects (\textit{i.e.} shape bias) and not on individual objects' peripheral features. This is inline with how human learns in general; our brain unconsciously focuses on the general shape of objects rather than superficial statistics of context. On the other hand, learning autonomously allows discovering invariant regularities which help generalization [[this sentence needs major revision. it's very vague]]. Inspired by these observations, we propose a learning framework to improve the learning performance of self-supervised methods by further hitching their learning process to shape bias. Using distinct modules, our method learns semantic and shape biased representations by integrating domain diversification and jigsaw puzzles. The first module enables the model to create a dynamic environment across arbitrary domains and provides a domain exploration vs. exploitation trade-off, while the second module allows it to explore this environment autonomously. The proposed framework is universally adaptable since it does not require prior knowledge of the domain of interest. We empirically evaluate the performance of our framework through extensive experiments on several domain generalization datasets, namely, PACS, Office-Home, VLCS, and Digits. Results show that the proposed method outperforms the other state-of-the-arts on most of the datasets.
\end{abstract}

==> introv0.tex <==
\section{Introduction}
Convolutional Neural Networks have achieved significant success in a wide variety of visual recognition tasks, demonstrating an excellent ability to learn the spatial structure of image data.
Despite the promising results, the performance of these models diminishes considerably when extending the same application to different environments.
This is due to the significant dependency of these models on large-scale annotated training data. However, available benchmarks cannot cover all of the real-world environmental conditions.
This imposes severe issues for many practical applications which are not restricted to a specific domain \cite{torralba2011unbiased}.

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=6.5cm]{assets/jigsaw1.jpg}
%	\end{center}
%	\caption{Superficial statistics of image, e.g., textures, can help solve jigsaw puzzles which leads to unfavorable biases of the network. We propose a learning framework which creates a controllable dynamic environment across arbitrary domains and enables the agent(model) to explore this environment autonomously.}%pls note that as it gets deeper, samples get further from their correct class
%	\label{figure1}
%\end{figure}

In order to alleviate \textit{domain shift} problem, several domain adaptation methods have been proposed.\cite{csurka2017domain}
Due to the cost of manually annotating target domain data, \textit{unsupervised domain  adaptation}, namely adapting a trained model to a new domain but without annotating the target data, has attracted a considerable amount of research.
Some works tried to tackle this problem by matching the distribution of source and target domains.
In these methods, the goal is to reduce the difference between covariance matrices of source and target domains.\cite{sun2016deep, morerio2017minimal}.
Similarly, \cite{roy2019unsupervised} proposed \textit{Domain-specific Whitening Transform} which computes domain-specific covariance matrices of intermediate
features by whitening the source and the target
features and projecting them into a common spherical distribution.

Another recent approach used for unsupervised domain adaptation, embeds domain-specific alignment layers, inspired by BatchNorm\cite{ioffe2015batch} layers, within the network.\cite{cariucci2017autodial, mancini2018boosting}
Another category of domain translation methods focuses on the appearance translation of source domain towards the target domain.
Since many image translation methods are imperfect, these approaches have severe drawbacks especially when there is a significant gap between source and target domains \cite{bousmalis2017unsupervised, hoffman2017cycada, russo2018source}.

Due to the fact that \textit{unsupervised representation learning} helps the model to learn label-invariant and high-level representation of data, they can improve generalizability as well as the robustness of the model \cite{carlucci2019domain, hendrycks2019using}. 
Furthermore, unsupervised representation learning can solve the lack of large-scale annotated benchmarks since a sheer volume of unlabeled data is publicly available. Subsequently, these methods are less susceptible to unfavorable biases of data \cite{torralba2011unbiased}.
Inspired by what mentioned above, \cite{carlucci2019domain} proposed a method capable of learning spatial co-location of image parts simultaneously with supervised learning. Moreover, they show that self-supervision can have a considerable impact on the generalizability of the model.

Although self-supervised methods learn general feature embeddings, one major question still remains; how much is the learned feature representation of these methods biased towards superficial statistics of image e.g., textures and local features?
Humans' biological visual system has a considerable robust performance against domain shifts. It is known that humans display shape bias when classifying new objects \cite{ritter2017cognitive, geirhos2018generalisation}. Numerous studies have tried to improve the shape bias property of deep neural networks \cite{hosseini2018assessing, geirhos2018imagenet}. \cite{geirhos2018imagenet} proves that CNNs are highly biased towards learning superficial characteristics e.g., textures rather than general shape of objects which is in clear contrast with the human visual system. Moreover, \cite{brendel2019approximating} shows that CNNs tend to classify an image based on local image features without taking into account their spatial structure.

In this work, we investigate the learned feature representation of self-supervised methods. We state that, though unsupervised representation learning is capable of learning a label-invariant and high-level representation of the image, it is severely biased to unfavorable and superficial statistics of the data. We use \textit{jigsaw puzzle}\cite{noroozi2016unsupervised} pretext task, same as \cite{carlucci2019domain}. We prove that context-based self-supervised methods are significantly biased to the texture and local features of the image.
In other words, we tackle the shape-bias property of unsupervised representation learning methods. A texture diversification method is used in order to enforce the model to solve jigsaw task based on the general shape of each object rather than local textures and superficial features. Thereupon, we propose a self-supervised learning system based on jigsaw task which enables the agent(model) to explore arbitrary domains during the training process.
Furthermore, an extensive analysis is conducted on domain exploration vs. exploitation trade-off, and the behavior of the model is discussed in each setting. 

Since self-supervised methods learn an invariant representation of the data, improving shape bias property, and unbiasing them from superficial statistics, enhances the generalizability of these models to a significant extent. To validate our work, we conduct extensive experiments on domain generalization benchmarks and illustrate that our method outperforms state-of-the-art works on domain generalization.
The contributions of this paper are as follows:
\begin{itemize}
	\item We analyze the dependency of unsupervised representation learning methods on textures as well as local features of image. 
	\item We structurize an unsupervised representation learning paradigm by integrating domain diversification and jigsaw puzzles pretext task.
	\item Through extensive experiments, we show that our method outperforms state-of-the-art methods on domain generalization. Furthermore, the robustness of our method against distortions is studied.
\end{itemize}

\begin{figure*}[h!]
	\begin{center}
		\includegraphics[width=16cm]{assets/model.jpg}
	\end{center}
	\caption{Illustration of our proposed framework. Our framework enables the model(Convnet) to learn from both ordered and shuffled images. Our framework consists of Domain Diversification followed by Exploration Controller modules which create a dynamic environment across arbitrary domains. Consequently, the model can explore this environment autonomously, which improves the shape bias property of the network to a significant extent.}%pls note that as it gets deeper, samples get further from their correct class
	\label{figure2}
\end{figure*}


==> introv1MH.tex <==
\section{Introduction}
Convolutional Neural Networks have achieved significant success in a wide variety of visual recognition tasks, demonstrating an excellent ability to learn the spatial structure of image data.
Despite the promising results, the performance of these models diminishes considerably when applied to environments different than training. This fragile phenomenon is known as \textit{domain shift}.
% and is well-studied in the literature
This is due to the significant dependency of these models on large-scale annotated datasets. This issue imposes severe issues toward practical applications of deep neural networks and their generalization to domains beyond their own training one \cite{torralba2011unbiased}.

%\begin{figure}[h!]
%	\begin{center}
%		\includegraphics[width=6.5cm]{assets/jigsaw1.jpg}
%	\end{center}
%	\caption{Superficial statistics of image, e.g., textures, can help solve jigsaw puzzles which leads to unfavorable biases of the network. We propose a learning framework which creates a controllable dynamic environment across arbitrary domains and enables the agent(model) to explore this environment autonomously.}%pls note that as it gets deeper, samples get further from their correct class
%	\label{figure1}
%\end{figure}

In order to alleviate \textit{domain shift} problem, several domain adaptation methods have been proposed \cite{csurka2017domain, pan2009survey, wang2018deep} [[needs a couple of more citation]]
Due to the cost of manually annotating target domain data, unsupervised domain adaptation, \textit{i.e.} adapting a trained model to a new target domain without annotating the target dataset, has been the foundation for a considerable amount of research.
Early works in this domain tackled the problem by learning to match the distribution of source and target domains \cite{sun2016deep, morerio2017minimal}.
In these methods, the goal is to reduce the difference between covariance matrices of source and target domains.
Similarly \cite{roy2019unsupervised} proposed Domain-specific Whitening Transform which computes domain-specific covariance matrices of intermediate
features by whitening the source and the target
features and projecting them into a common spherical distribution.\\

[[next two paragraphs focuses too much on related work without linking them to our method; move them to sec. 2 or link them to our idea. remember intro. is where you can catch or lose your reviewer!]]\\

Another recent approach used for unsupervised domain adaptation, embeds domain-specific alignment layers, inspired by BatchNorm\cite{ioffe2015batch} layers, within the network \cite{cariucci2017autodial,mancini2018boosting}
Another category of domain translation methods focuses on the appearance translation of source domain towards the target domain.
Since many image translation methods are imperfect, these approaches have severe drawbacks especially when there is a significant gap between source and target domains \cite{bousmalis2017unsupervised, hoffman2017cycada, russo2018source}.

Due to the fact that unsupervised representation learning helps the model to learn label-invariant and high-level representation of data, they can improve generalizability as well as the robustness of the model \cite{carlucci2019domain, hendrycks2019using}. 
Furthermore, unsupervised representation learning can solve the lack of large-scale annotated benchmarks since a sheer volume of unlabeled data is publicly available. Subsequently, these methods are less susceptible to unfavorable biases of data \cite{torralba2011unbiased}.
Inspired by what mentioned above, \cite{carlucci2019domain} proposed a method capable of learning spatial co-location of image parts simultaneously with supervised learning. Moreover, they show that self-supervision can have a considerable impact on the generalizability of the model.

Although self-supervised methods learn general feature embeddings, one major question is how much is the learned  representation by these methods biased towards superficial statistics of image \textit{e.g.}, textures and local features?\\

[[this paragraph about human is wandering around like a youtube ad. move it to more appropriate place]]\\

Humans' biological visual system has a considerable robust performance against domain shifts. It is known that humans display shape bias when classifying new objects \cite{ritter2017cognitive, geirhos2018generalisation}. \\

[[too much related work again. try to pitch your own method]]\\

Numerous studies have tried to improve the shape bias property of deep neural networks \cite{hosseini2018assessing, geirhos2018imagenet}. \cite{geirhos2018imagenet} proves that CNNs are highly biased towards learning superficial characteristics e.g., textures rather than general shape of objects which is in clear contrast with the human visual system. Moreover, \cite{brendel2019approximating} shows that CNNs tend to classify an image based on local image features without taking into account their spatial structure.

In this work, we investigate the learned feature representation of self-supervised methods. We state that, though unsupervised representation learning is capable of learning a label-invariant and high-level representation of the image, it is severely biased to unfavorable and superficial statistics of the data. We use jigsaw puzzle \cite{noroozi2016unsupervised} pretext task, same as \cite{carlucci2019domain}[[to do what? complete the sentence]] . We show [[show not prove. we don't use theory stuff]] that context-based self-supervised methods are significantly biased to the texture and local features of the image.

To remedy it, a novel shape-biased framework for self-supervised methods is proposed as a means to learn more generalized representation and reduce domain shift problem. A texture diversification method is used in order to enforce the model to solve jigsaw task based on the general shape of each object rather than local textures and superficial features. Thereupon, we propose a self-supervised learning system based on jigsaw task which enables the model to explore arbitrary domains during the training process.
Furthermore, an extensive analysis is conducted on domain exploration vs. exploitation trade-off, and the behavior of the model is discussed in each setting. 

Since self-supervised methods learn an invariant representation of the data, improving shape bias property, and unbiasing them from superficial statistics, enhances the generalizability of these models to a significant extent. Finally to evaluate [[validate means you had it in mind and then tried to make experiments show it, too! have a bad impression on reviewer]] our work, we conduct extensive experiments on domain generalization benchmarks and illustrate that our method outperforms state-of-the-art works on domain generalization.
To summarize the contribution of this paper is manifold:
\begin{itemize}
	\item We analyze the dependency of unsupervised representation learning methods on textures as well as local features of image. 
	\item We structurize an unsupervised representation learning paradigm by integrating domain diversification and jigsaw puzzles pretext task.
	\item Through extensive experiments, we show that our method outperforms state-of-the-art methods on domain generalization. Furthermore, the robustness of our method against distortions is studied.
\end{itemize}

\begin{figure*}[h!]
	\begin{center}
		\includegraphics[width=16cm]{assets/model.jpg}
	\end{center}
	\caption{Illustration of our proposed framework. Our framework enables the model(Convnet) to learn from both ordered and shuffled images. Our framework consists of Domain Diversification followed by Exploration Controller modules which create a dynamic environment across arbitrary domains. Consequently, the model can explore this environment autonomously, which improves the shape bias property of the network to a significant extent.}%pls note that as it gets deeper, samples get further from their correct class
	\label{figure2}
\end{figure*}


==> methodv0.tex <==
\section{Methodology}
\subsection{Overview and Motivation}
It is known that the human visual system generally displays shape bias.
On the other hand, humans seem to rely crucially on learning autonomously. As a matter of fact, the human visual system adaptability relies on both of the aforementioned approaches.
Since unsupervised representation learning methods are label-invariant, they can help the model to discover invariances and regularities that help to generalize \cite{carlucci2019domain}.
However, the learned feature representation in these methods is highly dependent on the pretext task e.g., jigsaw puzzles which might cause unfavorable biases in learned feature representation. In order to solve this task, the model can also use superficial statistics which severely harm shape bias property as well as the generalizability of the model.


We propose a learning paradigm to improve the shape bias property of unsupervised representation learning by alleviating unfavorable biases to superficial statistics of the image.
Our framework is based on domain diversification and self-supervision together, which allows the model to be free from a single static domain. In other words, the agent(model) is able to autonomously explore a dynamic environment across arbitrary domains in an effort of learning domain invariant and shape biased characteristics of the problem.
Also, we demonstrate that exploration vs. exploitation trade-off can help the model learn useful and unbiased representations.
Our method has two major modules, Domain Diversification followed by exploration vs. exploitation controller and unsupervised representation learning by solving jigsaw puzzles. In the following, we describe each module in detail, and finally, a domain invariant learning framework is introduced. Figure \ref{figure2} demonstrates conceptual description of our method.

\subsection{Jigsaw Puzzles for Domain Generalization}
Previous work \cite{carlucci2019domain} has shown the efficiency of solving jigsaw puzzles on learning a general representation of the image. We use the same approach as the baseline of our framework.
This module consists of a convolutional feature extractor and two fully connected parts.
Consider $x$ as the input of the network, $y$ as the correct label, and $\theta_f$, $\theta_c$, $\theta_j$ as parameters of convolutional feature extractor, cross-entropy classifier, jigsaw classifier respectively.
The objective of the first fully-connected module is to minimize the cross-entropy loss between ground-truth label $y$ and predicted label by the model parameterized by $\theta_f$ and $\theta_c$. This module, as well as the feature extractor, are trained through
\begin{equation}
\underset{\theta_f, \theta_c}{argmin}
\sum\limits_{j=1}\limits^{N_i}
L_c (h(x_j^i | \theta_f, \theta_c), y_j^i)
\end{equation}

The objective of the second module is to predict permutation set in a decomposed image of $n \times n$ grid of patches being randomly shuffled. The overall number of possible permutations is $n^2!$, however, similar to \cite{carlucci2019domain}, a set of P elements is selected following the Hamming distance-based algorithm presented in \cite{noroozi2016unsupervised}. This module, as well as the feature extractor, are trained through
\begin{equation}
\underset{\theta_f, \theta_j}{argmin}
\sum\limits_{k=1}\limits^{K_i}
L_j (h(z_k^i | \theta_f, \theta_j), p_k^i)
\end{equation}
where $z_k^i$ indicates the decomposed samples and $p_k^i$ the corresponding permutation index.

\subsection{Domain Diversification}
Domain Diversification is a method which diversifies the source domain by intentionally generating distinctive domain discrepancy through these domain shifters.
Without harming general shape of the object, the domain of each jigsaw puzzle tile is shifted arbitrarily.
Consequently, superficial statistics of the image like textures, have no benefits for solving the pretext task. Thus, the model is enforced to extract features relevant to the general shape of each object. As a result, the self-supervised model will be biased to the high-level shape of objects rather than local textures and background.

Due to the imperfect performance of domain-shifters, they can cause issues when directly used for domain adaptation problems. However, our framework is utilized by domain diversification to create a dynamic environment in which the self-supervised module is enforced to learn domain-invariant representations. So, we use a modification of \textit{Adaptive Instance Normalization} method due to its high speed and acceptable performance.
%Since some of the hyper-parameters of AdaIN have a significant impact on not only exploration vs. exploitation trade-off but also the overall performance of our framework, we briefly discuss this method. For further details, we refer the reader to \cite{huang2017arbitrary}.
Consider $x^s$ as the feature representation of source data and $x^t$ as the feature representation of an arbitrary target domain. In general, style transfer methods align the channel-wise mean and variance of $x^s$ to match those of $x^t$.
\begin{equation}
	\textnormal{AdaIN}(x^s, x^t) = \sigma(x^t)(\frac{x^s - \mu(x^s)}{\sigma(x^s)}) +
	\mu(x^s)
\end{equation}\label{eq3}
as one can see, AdaIN simply scales the normalized content input with $\sigma(x^t)$, and shift it with $\mu(x^t)$. It is crucial to keep the overall shape of each tile intact. The loss function below matches the style of source image to the target image.
\begin{multline}
L_s(t, s) = \sum_{i = 1}^{N}\|\mu(\phi_i(g(t))) - \mu(\phi_i(s))\|_2 +\\ 
\sum_{i = 1}^{N}\|\sigma(\phi_i(g(t))) - \sigma(\phi_i(s))\|_2
\end{multline}
where $\phi$ denotes a layer in VGG-19 used to computer the style loss. Meanwhile, adjacent tiles should be of distant domains in order to enforce the self-supervised model learn shape biased representations.
Moreover, since the texture of each tile is changed randomly in each iteration of training, the superficial statistics of the image have no benefits for solving the jigsaw puzzle. To redeem this problem, we add an objective function to enforce the model diversify adjacent tiles without harming the shape of object.
\begin{equation}
L_{j} = \sum_{j = 2}^{K - 1}L_s(z_k, z_{k-1}) + L_s(z_k, z_{k+1}) 
\end{equation}
where $K$ is the number of jigsaw tiles and $z_k$ indicates the decomposed samples . A pretrained VGG-19 is used to compute the loss function:
\begin{equation}
L = L_c + \lambda L_s - \tau L_{j}
\end{equation}\label{eq5}
which is a weighted combination of the content loss and style losses where $L_c$ is
\begin{equation}
L_c = \|f(g(t)) - t\|_2
\end{equation}\label{eq6}
In order to keep the overall shape of the object intact, $\lambda$ and $\tau$ parameters should be chosen smaller compared to style transfer problems.
Finally, the output of translation module is computed as:
\begin{equation}
	T({x^s}, {x^t}, \gamma) = g((1 - \gamma)f(x^s) + \gamma \textnormal{AdaIN}(f(x^s), f(x^t)))
\end{equation}\label{eq7}
where $f$ is the pretrained VGG19 encoder, $g$ is the trained decoder using Eq \ref{eq3}, and $\gamma$ allows content-style trade-off at test time.

%\vspace{2mm}
%\noindent
%\textbf{Structured Framework}\quad 
\subsection{Structured Framework}\label{sec_framework}
In this section, we structurize our learning paradigm by integrating Domain Diversification and solving jigsaw puzzles into a framework. As previously discussed, though self-supervised methods learn general and high-level representation of data, they can be highly biased to superficial statistics of the image e.g., textures and local features. The objective of our work is to create a dynamic environment across domains for the agent(model) to autonomously learn texture-invariant and shape-biased statistics of the data.
To achieve this goal, we randomly shift each jigsaw tile to an arbitrary domain. Subsequently, the superficial context and texture of the piles have no advantage for solving the pretext task; thus, the model is enforced to rely on the overall shape of each object to solve the task. The overall objective function of the framework can be written as follows:
\begin{multline}
	\underset{\theta_f, \theta_c, \theta_j}{argmin}
	\sum\limits_{i=1}\limits^{N}
	L_c (h(x_i | \theta_f, \theta_c), y_i)
	 + \\
	\sum\limits_{k=1}\limits^{K}
	\alpha L_j (h(D(z_k, \rho) | \theta_f, \theta_j), p_k)
\end{multline}
Here, $N$ is the number of labeled instances, $z_k$ indicates the recomposed samples for jigsaw task, $\alpha$ is the weight parameter for jigsaw loss, $\rho$ is the domain shift probability parameter, and $D$ stands for domain diversification model trained using Eq\ref{eq5}.

\vspace{2mm}
\noindent
\textbf{Exploration vs Exploitation Trade-off}\quad \\
Our framework has four important hyper-parameters. Two of which, namely $\alpha$ and $\beta$, are related to solving jigsaw puzzles \cite{carlucci2019domain}. The $\alpha$ parameter, as mentioned before, controls the significance of jigsaw loss on the overall objective function. The $\beta$ parameter defines the ratio between ordered and shuffled images.

Two other parameters, namely $\gamma$ and $\rho$, are highly correlated with exploration vs. exploitation trade-off.
The $\rho$ parameter indicates the probability of domain shift, in other words, exploration weight. For instance, $\rho = 0.7$ means that for each batch, 70\% of the shuffled images have arbitrarily shifted patches. On the other hand, $\gamma$ (Eq. \ref{eq5}) defines the magnitude of texture translation; in other words, the step size towards arbitrary domain at exploration time.
These two parameters enable the model to explore a dynamic environment across arbitrary domains autonomously.
In the following section, we conduct extensive analysis on the impact of these parameters on the learned feature representation of the network.

